An Analysis of Source-Side Grammatical Errors in NMT

The quality of Neural Machine Translation (NMT) has been shown to significantly degrade when confronted with source-side noise. We present the first large-scale study of state-of-the-art English-to-German NMT on real grammatical noise, by evaluating on several Grammar Correction corpora. We present methods for evaluating NMT robustness without true references, and we use them for extensive analysis of the effects that different grammatical errors have on the NMT output. We also introduce a technique for visualizing the divergence distribution caused by a source-side error, which allows for additional insights.

==> related.tex <==
\begin{table*}[t]
    \centering
    \begin{tabular}{lc|p{4cm}|cc}
    \toprule
        Work & Errors & Noise Types & NMT level & Languages \\
    \midrule
        \cite{heigold2017robust} & synthetic & character swaps, character flips, word scrambling & char, BPE & De$\rightarrow$En\\
    \midrule
        \cite{sperbertoward} & synthetic & ASR errors & word & Es$\rightarrow$En\\
    \midrule
        \multirow{4}{*}{\cite{belinkov2017synthetic}} & synthetic & character swap, middle scramble, full scramble, keyboard typo & \multirow{2}{*}{char, BPE} & \multirow{2}{*}{Fr,De,Cz$\rightarrow$En} \\
        & semi-natural & word substitutions & \\ 
    \midrule
        \multirow{4}{*}{this work} & semi-natural & grammar errors: article, preposition, noun number, verb agreement & \multirow{2}{*}{BPE} & \multirow{2}{*}{En$\rightarrow$Es}\\
        & natural & JFLEG corpus & \\
    \bottomrule
    \end{tabular}
    \caption{Previous work on evaluating the effect of noise in NMT systems. Character swaps refer to neighboring character reordering (e.g. noise$\rightarrow$nosie), while character flips refer to character substitutions (e.g. noise$\rightarrow$noiwe).}
    \label{tab:previous}
\end{table*}

==> related_work.tex <==
\section{Related Work}

The effect of noise in NMT was recently studied by \citet{khayrallah-koehn:2018:WNMT}, who explored noisy situations during training due to web-crawled data. 
This type of noise includes misaligned, mistranslated, or untranslated sentences which, when used during training, significantly degrades the performance of NMT. 
Unlike our work, they primarily focus on a setting where the training set is noisy but the test set is clean.

In addition, \citet{heigold2017robust} evaluated the robustness of word embeddings against word scrambling noise, and showed that performance in downstream tasks like POS-tagging and MT is especially hurt. 
\citet{sakaguchi2017robsut} 
studied word scrambling and the \emph{Cmabrigde Uinervtisy (Cambridge University) effect}, where humans are able to understand the meaning of sentences with scrambled words,
performing word recognition (word level spelling correction) with a semi-character RNN system.

Focusing only on character-level NMT models, \citet{belinkov2017synthetic} showed that they exhibit degraded performance when presented with noisy test examples (both artificial and natural occurring noise). 
In line with our findings, they also showed that slightly better performance can be achieved by training on data artificially induced with the same kind of noise as the test set.

\citet{sperbertoward} proposed a noise-introduction system reminiscent of WER, based on insertions, deletions, and substitutions. An NMT system tested on correct transcriptions achieves a BLEU score of $55$ (4 references), but tested on the ASR transcriptions it only achieves a BLEU score of $35.7$. By introducing similar noise in the training data, they were able to make the NMT system slightly more robust. Interestingly, they found that the optimal amount of noise on the training data is smaller than the amount of noise on the test data.

The notion of linguistically plausible corruption is also explored by \citet{li2017robust}, who created adversarial examples with syntactic and semantic noise (reordering and word substitutions respectively). When training with these noisy datasets, they obtained better performance on several text classification tasks. Furthermore, in accordance with our results, their best system is the one that combines different types of noise.

We present a summary of relevant previous work in Table~\ref{tab:previous}. 
\emph{Synthetic} errors refer to noise introduced according an artificially created distribution, and \emph{natural} errors refer to actual errorful text produced by humans. As for \emph{semi-natural}, it refers to either noise introduced according to a distribution learned from data (as in our work), or to errors that are learned from data but introduced according to an artificial distribution (as is part of the work of \citet{belinkov2017synthetic}).

We consider our work to be complementary to the works of \citet{heigold2017robust,belinkov2017synthetic}, and \citet{sperbertoward}. However, there are several important differences:
\input{related.tex}
\begin{enumerate}[nolistsep]
    \item \citet{belinkov2017synthetic} and \citet{sperbertoward} train their NMT systems on fairly small datasets: 235K (Fr-En), 210K (De-En), 122K (Cz-En), and 138K sentences (Es-En) respectively. Even though they use systems like Nematus \cite{sennrich2017nematus} or XNMT \cite{neubig2018xnmt} which generally achieve nearly SOTA results, it is unclear whether their results generalize to larger training data. In contrast, we train our system on almost 2M sentences.
    
    \item All three systems introduce somewhat unrealistic amounts of noise in the data. The natural noise of \citet{belinkov2017synthetic} consists of word substitutions based on Wikipedia errors or corrected essays (in the Czech case) but they substitute all possible correct words with their erroneous version, ending up with datasets with more than $40\%$ of the tokens being noisy. For that reason, we refer to it as \emph{semi-natural} noise in Table~\ref{tab:previous}.  Meanwhile, \citet{sperbertoward} test on the outputs of an ASR system that has a WER of $41.3\%$. For comparison, in the \jfleg datasets, we calculated that only about $3.5\%$--$5\%$ of the tokens are noisy -- the average Levenshtein distance of a corrected reference and its noisy source is 13 characters.
    
    \item The word scrambling noise, albeit interesting, could not be claimed to be applicable to realistic scenarios, especially when applied to all words in a sentence. 
    The solution \citet{belinkov2017synthetic} suggested and \citet{sperbertoward} discussed is a character- or spelling-aware model for producing word- or subword-level embeddings. We suspect that such a solution would indeed be appropriate for dealing with typos and other character-level noise, but not for more general grammatical noise. 
    Our method could potentially be combined with GloVe \cite{pennington2014glove} or fastText \cite{bojanowski2017enriching} embeddings that can deal with slight spelling variations, but we leave this for future work.
\end{enumerate}

On the other side, Grammar Error Correction has been extensively studied, with significant incremental advances made recently by treating GEC as an MT task: 
among others, \citet{junczysdowmunt-grundkiewicz:2016:EMNLP2016} used phrased-based MT, \citet{ji-EtAl:2017:Long} used hybrid character-word neural sequence-to-sequence systems, \citet{sakaguchi2017grammatical} used reinforcement learning, and \citet{dowmunt2018etal} combined several techniques with NMT to achieve the current state-of-the-art.
Synthetic errors for training GEC systems have also been studied and applied with mixed success \cite{rozovskaya2010generating,rozovskaya2014illinois,xie2016neural}, while more recently \citet{xie2018noising} used backtranslation techniques for adding synthetic noise useful for GEC.



==> robustness.tex <==
\begin{table*}[t]
    \centering
    \begin{tabular}{c|cc|cc|cc|cc|cc}
    \toprule
        \multirow{2}{*}{Training} &  \multicolumn{10}{c}{a) WMT Test Set}\\
          & \drop & $\Delta$ & \art & $\Delta$  & \prep & $\Delta$  & \nn & $\Delta$  &\sva & $\Delta$  \\
        \midrule
        \clean & 75.1 & \xt{+1.9}& 80.3 &\xt{+0.9} & 83.7 &\xt{+0.3} & 75.1 & \xt{+3.3} & 87.2 &\xt{-0.1} \\
        \mixd & 77.0 && 81.2 && 84.0 && 78.4 && 87.1 \\
        \midrule\midrule
        & \multicolumn{10}{c}{ b) \jfleges Dev Set} \\
        & \textsc{cor0} & $\Delta$ & \textsc{cor1} & $\Delta$  & \textsc{cor2} & $\Delta$  & \textsc{cor3} & $\Delta$  & \textsc{all-cor} & $\Delta$  \\
        \cmidrule{2-11}
        \clean & 55.2 & \xt{+0}
        & 53.5 & \xt{+0.8} & 59.8 & \xt{+0.5} & 62.4 & \xt{+1.8} & 78.1 & \xt{+1.4} \\
        \mixd & 55.2 && 54.2 && 60.3 && 64.2 && 79.5 & \\
        \midrule
        & \multicolumn{10}{c}{c) \jfleges Test Set} \\
        & \textsc{cor0} & $\Delta$  & \textsc{cor1} & $\Delta$  & \textsc{cor2} & $\Delta$  & \textsc{cor3} & $\Delta$  & \textsc{all-cor} & $\Delta$  \\
        \cmidrule{2-11}
        \clean & 59.7 & \xt{+2.8} & 61.3 & \xt{+2.8} & 57.9 & \xt{+2.2} & 52.9 & \xt{+3.1} & 74.9 & \xt{+2.8}\\
        \mixd  & 62.9 && 64.1 && 60.1 && 56.0 && 77.7 & \\
    \bottomrule
    \end{tabular}
    \caption{\emph{a)}: Robustness on each type of error, computed with BLEU against the produced translation of the clean sentence. We find that our proposed solution (\textsc{mix-both}) is generally more robust.\\
    \emph{b,c)}: Robustness against \jfleg correction sets. For \jfleges \textsc{all-cor} we use multi-reference BLEU against the translations of all four \jfleges references. Again, \mixd outperforms the \clean model.}
    \label{tab:robust1}
\end{table*}

==> trdata.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{cccc}
    \toprule
        \multirow{2}{*}{Dataset} & \multicolumn{3}{c}{Percentage of Errors} \\
         & Train & Dev & Test \\
    \midrule
        sentences & 2M & 3K & 3K \\
        words & 55M & 74K & 73K \\
    \midrule
        \drop & 100\% & 100\% & 100\% \\
        \art & 96.4\% & 98.4\% & 99.8\% \\
        \prep & 95.7\% & 95.9\% & 98.4\% \\
        \nn & 94.5\% & 91.0\% & 98.6\% \\
        \sva & 93.1\% & 81.9\% & 82.0\% \\
    \midrule
        \dropd & 50\% & 50\% & -- \\
        \artd & 48.2\% & 49.1\% & -- \\
        \prepd & 47.8\% & 47.9\% & -- \\
        \nnd & 47.3\% & 45.5\% & -- \\
        \svad & 46.5\% & 41.0\% & -- \\
    \midrule
        %WMT-\mixd & 48.1\% & 47.7\% & -- \\
        \mixall & 39.9\% & 38.9\% & -- \\
    \bottomrule
    \end{tabular}
    \caption{Statistics on the original and synthetic En-Es datasets. Each (synthetic) sentence has exactly one introduced error, wherever possible.  
    \textsc{clean+[error]} is the concatenation of the \textsc{[error]} with the original clean dataset, while
    \mixall includes six versions of each training sentence, one without errors and one for each error.}
    %WMT-\mixd includes two versions of each training sentence, one without and one with an error.}
    \label{tab:synthdata}
\end{table}
